Towards Black-box Attacks on Deep Learning Apps

Deep learning is a powerful weapon to boost application performance in many fields, including face recognition, object detection, image classification, natural language understanding, and recommendation system. With the rapid increase in the computing power of mobile devices, developers can embed deep learning models into their apps for building more competitive products with more accurate and faster responses. Although there are several works about adversarial attacks against deep learning models in mobile apps, they all need information about the models' internals (i.e., structures, weights) or need to modify the models. In this paper, we propose an effective black-box approach by training a substitute model to spoof the deep learning system inside the apps. To evaluate our approach, we select 10 real-world deep-learning apps with high popularity from Google Play to perform black-box adversarial attacks. Through the study, we find three factors that can influence the performance of attacks. Our approach can reach a relatively high attack success rate of 66.60% on average. Compared with other adversarial attacks on mobile deep learning models, in terms of the average attack success rates, our approach outperforms counterparts by 27.63%.

==> sec/motivating-example.tex <==
\section{Motivating Example}
% case study 
% 真实的故事 场景 说明 你的方法 
% App1  ---》 Teacher Studenter 
% (1) student 的训练数据哪里来 
% (2) 

% （3）可以成功攻击  （由现象 有截图 ---》直观的方式 ）

% 图1 （对抗样本）和原图 
% 图2  结果


